Development of a data overflow protection system for Super-Kamiokande to maximize data from nearby supernovae

Neutrinos from very nearby supernovae, such as Betelgeuse, are expected to generate more than ten million events over 10\,s in Super-Kamokande (SK). At such large event rates, the buffers of the SK analog-to-digital conversion board (QBEE) will overflow, causing random loss of data that is critical for understanding the dynamics of the supernova explosion mechanism. In order to solve this problem, two new DAQ modules were developed to aid in the observation of very nearby supernovae. The first of these, the SN module, is designed to save only the number of hit PMTs during a supernova burst and the second, the Veto module, prescales the high rate neutrino events to prevent the QBEE from overflowing based on information from the SN module. In the event of a very nearby supernova, these modules allow SK to reconstruct the time evolution of the neutrino event rate from beginning to end using both QBEE and SN module data. This paper presents the development and testing of these modules together with an analysis of supernova-like data generated with a flashing laser diode. We demonstrate that the Veto module successfully prevents DAQ overflows for Betelgeuse-like supernovae as well as the long-term stability of the new modules. During normal running the Veto module is found to issue DAQ vetos a few times per month resulting in a total dead time less than 1\,ms, and does not influence ordinary operations. Additionally, using simulation data we find that supernovae closer than 800~pc will trigger Veto module resulting in a prescaling of the observed neutrino data.

==> affiliations.tex <==
\newcommand{\AFFicrr}{\affiliation{Kamioka Observatory, Institute for Cosmic Ray Research, University of Tokyo, Kamioka, Gifu 506-1205, Japan}}
\newcommand{\AFFkashiwa}{\affiliation{Research Center for Cosmic Neutrinos, Institute for Cosmic Ray Research, University of Tokyo, Kashiwa, Chiba 277-8582, Japan}}
\newcommand{\AFFicrronly}{\affiliation{Institute for Cosmic Ray Research, University of Tokyo, Kashiwa, Chiba 277-8582, Japan}}
\newcommand{\AFFipmu}{\affiliation{Kavli Institute for the Physics and
Mathematics of the Universe (WPI), The University of Tokyo Institutes for Advanced Study,
University of Tokyo, Kashiwa, Chiba 277-8583, Japan }}
\newcommand{\AFFmad}{\affiliation{Department of Theoretical Physics, University Autonoma Madrid, 28049 Madrid, Spain}}
\newcommand{\AFFubc}{\affiliation{Department of Physics and Astronomy, University of British Columbia, Vancouver, BC, V6T1Z4, Canada}}
\newcommand{\AFFbu}{\affiliation{Department of Physics, Boston University, Boston, MA 02215, USA}}
\newcommand{\AFFuci}{\affiliation{Department of Physics and Astronomy, University of California, Irvine, Irvine, CA 92697-4575, USA }}
\newcommand{\AFFcsu}{\affiliation{Department of Physics, California State University, Dominguez Hills, Carson, CA 90747, USA}}
\newcommand{\AFFcnm}{\affiliation{Institute for Universe and Elementary Particles, Chonnam National University, Gwangju 61186, Korea}}
\newcommand{\AFFduke}{\affiliation{Department of Physics, Duke University, Durham NC 27708, USA}}
\newcommand{\AFFfukuoka}{\affiliation{Junior College, Fukuoka Institute of Technology, Fukuoka, Fukuoka 811-0295, Japan}}
\newcommand{\AFFgifu}{\affiliation{Department of Physics, Gifu University, Gifu, Gifu 501-1193, Japan}}
\newcommand{\AFFgist}{\affiliation{GIST College, Gwangju Institute of Science and Technology, Gwangju 500-712, Korea}}
\newcommand{\AFFuh}{\affiliation{Department of Physics and Astronomy, University of Hawaii, Honolulu, HI 96822, USA}}
\newcommand{\AFFicl}{\affiliation{Department of Physics, Imperial College London , London, SW7 2AZ, United Kingdom }}
\newcommand{\AFFkek}{\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba, Ibaraki 305-0801, Japan }}
\newcommand{\AFFkobe}{\affiliation{Department of Physics, Kobe University, Kobe, Hyogo 657-8501, Japan}}
\newcommand{\AFFkyoto}{\affiliation{Department of Physics, Kyoto University, Kyoto, Kyoto 606-8502, Japan}}
\newcommand{\AFFliv}{\affiliation{Department of Physics, University of Liverpool, Liverpool, L69 7ZE, United Kingdom}}
\newcommand{\AFFmiyagi}{\affiliation{Department of Physics, Miyagi University of Education, Sendai, Miyagi 980-0845, Japan}}
\newcommand{\AFFnagoya}{\affiliation{Institute for Space-Earth Environmental Research, Nagoya University, Nagoya, Aichi 464-8602, Japan}}
\newcommand{\AFFkmi}{\affiliation{Kobayashi-Maskawa Institute for the Origin of Particles and the Universe, Nagoya University, Nagoya, Aichi 464-8602, Japan}}
\newcommand{\AFFpol}{\affiliation{National Centre For Nuclear Research, 02-093 Warsaw, Poland}}
\newcommand{\AFFsuny}{\affiliation{Department of Physics and Astronomy, State University of New York at Stony Brook, NY 11794-3800, USA}}
\newcommand{\AFFokayama}{\affiliation{Department of Physics, Okayama University, Okayama, Okayama 700-8530, Japan }}
\newcommand{\AFFosaka}{\affiliation{Department of Physics, Osaka University, Toyonaka, Osaka 560-0043, Japan}}
\newcommand{\AFFox}{\affiliation{Department of Physics, Oxford University, Oxford, OX1 3PU, United Kingdom}}
\newcommand{\AFFqmul}{\affiliation{School of Physics and Astronomy, Queen Mary University of London, London, E1 4NS, United Kingdom}}
\newcommand{\AFFregina}{\affiliation{Department of Physics, University of Regina, 3737 Wascana Parkway, Regina, SK, S4SOA2, Canada}}
\newcommand{\AFFseoul}{\affiliation{Department of Physics, Seoul National University, Seoul 151-742, Korea}}
\newcommand{\AFFsheff}{\affiliation{Department of Physics and Astronomy, University of Sheffield, S3 7RH, Sheffield, United Kingdom}}
\newcommand{\AFFshizuokasc}{\affiliation{Department of Informatics in
Social Welfare, Shizuoka University of Welfare, Yaizu, Shizuoka, 425-8611, Japan}}
\newcommand{\AFFstfc}{\affiliation{STFC, Rutherford Appleton Laboratory, Harwell Oxford, and Daresbury Laboratory, Warrington, OX11 0QX, United Kingdom}}
\newcommand{\AFFskk}{\affiliation{Department of Physics, Sungkyunkwan University, Suwon 440-746, Korea}}
%\newcommand{\AFFtokyo}{\affiliation{The University of Tokyo, Bunkyo, Tokyo 113-0033, Japan }}
\newcommand{\AFFtodai}{\affiliation{Department of Physics, University of Tokyo, Bunkyo, Tokyo 113-0033, Japan }}
\newcommand{\AFFtit}{\affiliation{Department of Physics,Tokyo Institute of Technology, Meguro, Tokyo 152-8551, Japan }}
\newcommand{\AFFtus}{\affiliation{Department of Physics, Faculty of Science and Technology, Tokyo University of Science, Noda, Chiba 278-8510, Japan }}
\newcommand{\AFFtoronto}{\affiliation{Department of Physics, University of Toronto, ON, M5S 1A7, Canada }}
\newcommand{\AFFtriumf}{\affiliation{TRIUMF, 4004 Wesbrook Mall, Vancouver, BC, V6T2A3, Canada }}
\newcommand{\AFFtokai}{\affiliation{Department of Physics, Tokai University, Hiratsuka, Kanagawa 259-1292, Japan}}
\newcommand{\AFFtsinghua}{\affiliation{Department of Engineering Physics, Tsinghua University, Beijing, 100084, China}}
\newcommand{\AFFynu}{\affiliation{Department of Physics, Yokohama National University, Yokohama, Kanagawa, 240-8501, Japan}}
\newcommand{\AFFllr}{\affiliation{Ecole Polytechnique, IN2P3-CNRS, Laboratoire Leprince-Ringuet, F-91120 Palaiseau, France }}
\newcommand{\AFFbari}{\affiliation{ Dipartimento Interuniversitario di Fisica, INFN Sezione di Bari and Universit\`a e Politecnico di Bari, I-70125, Bari, Italy}}
\newcommand{\AFFnapoli}{\affiliation{Dipartimento di Fisica, INFN Sezione di Napoli and Universit\`a di Napoli, I-80126, Napoli, Italy}}
\newcommand{\AFFroma}{\affiliation{INFN Sezione di Roma and Universit\`a di Roma ``La Sapienza'', I-00185, Roma, Italy}}
\newcommand{\AFFpadova}{\affiliation{Dipartimento di Fisica, INFN Sezione di Padova and Universit\`a di Padova, I-35131, Padova, Italy}}
\newcommand{\AFFkeio}{\affiliation{Department of Physics, Keio University, Yokohama, Kanagawa, 223-8522, Japan}}
\newcommand{\AFFwinnipeg}{\affiliation{Department of Physics, University of Winnipeg, MB R3J 3L8, Canada }}
\newcommand{\AFFkcl}{\affiliation{Department of Physics, King's College London, London, WC2R 2LS, UK }}
\newcommand{\AFFwarwick}{\affiliation{Department of Physics, University of Warwick, Coventry, CV4 7AL, UK }}
\newcommand{\AFFral}{\affiliation{Rutherford Appleton Laboratory, Harwell, Oxford, OX11 0QX, UK }}
\newcommand{\AFFwu}{\affiliation{Faculty of Physics, University of Warsaw, Warsaw, 02-093, Poland }}
\newcommand{\AFFbcit}{\affiliation{Department of Physics, British Columbia Institute of Technology, Burnaby, BC, V5G 3H2, Canada }}
\newcommand{\AFFtohoku}{\affiliation{Department of Physics, Faculty of Science, Tohoku University, Sendai, Miyagi, 980-8578, Japan }}
\newcommand{\AFFicise}{\affiliation{Institute For Interdisciplinary Research in Science and Education, ICISE, Quy Nhon, 55121, Vietnam }}
\newcommand{\AFFilance}{\affiliation{ILANCE, CNRS - University of Tokyo International Research Laboratory, Kashiwa, Chiba 277-8582, Japan}}
\newcommand{\AFFibs}{\affiliation{Institute for Basic Science (IBS), Daejeon, 34126, Korea}}

==> ptep_authors.tex <==
\newcommand{\AFFicrr}{1}
\newcommand{\AFFkashiwa}{2}
\newcommand{\AFFicrrkashiwa}{3}
\newcommand{\AFFmad}{4}
\newcommand{\AFFbu}{5}
\newcommand{\AFFbcit}{6}
\newcommand{\AFFuci}{7}
\newcommand{\AFFcsu}{8}
\newcommand{\AFFcnm}{9}
\newcommand{\AFFduke}{10}
\newcommand{\AFFllr}{11}
\newcommand{\AFFfukuoka}{12}
\newcommand{\AFFgifu}{13}
\newcommand{\AFFgist}{14}
\newcommand{\AFFuh}{15}
\newcommand{\AFFicl}{16}
\newcommand{\AFFbari}{17}
\newcommand{\AFFnapoli}{18}
\newcommand{\AFFpadova}{19}
\newcommand{\AFFroma}{20}
\newcommand{\AFFkeio}{21}
\newcommand{\AFFkek}{22}
\newcommand{\AFFkcl}{23}
\newcommand{\AFFkobe}{24}
\newcommand{\AFFkyoto}{25}
\newcommand{\AFFliv}{26}
\newcommand{\AFFmiyagi}{27}
\newcommand{\AFFnagoya}{28}
\newcommand{\AFFkmi}{29}
\newcommand{\AFFpol}{30}
\newcommand{\AFFsuny}{31}
\newcommand{\AFFokayama}{32}
\newcommand{\AFFosaka}{33}
\newcommand{\AFFox}{34}
\newcommand{\AFFqmul}{35}
\newcommand{\AFFral}{36}
\newcommand{\AFFseoul}{37}
\newcommand{\AFFsheff}{38}
\newcommand{\AFFshizuokasc}{39}
\newcommand{\AFFstfc}{40}
\newcommand{\AFFskk}{41}
\newcommand{\AFFtokai}{42}
\newcommand{\AFFtokyo}{43}
\newcommand{\AFFtodai}{44}
\newcommand{\AFFipmu}{45}
\newcommand{\AFFtit}{46}
\newcommand{\AFFtus}{47}
\newcommand{\AFFtoronto}{48}
\newcommand{\AFFtriumf}{49}
\newcommand{\AFFtsinghua}{50}
\newcommand{\AFFwu}{51}
\newcommand{\AFFwarwick}{52}
\newcommand{\AFFwinnipeg}{53}
\newcommand{\AFFynu}{54}

\author{
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%ICRR
\name{A.~Orii}{\AFFicrr},
\name{K.~Abe}{\AFFicrr,\AFFipmu},
\name{C.~Bronner}{\AFFicrr},
\name{Y.~Hayato}{\AFFicrr,\AFFipmu},
\name{M.~Ikeda}{\AFFicrr},
\name{S.~Imaizumi}{\AFFicrr},
\name{H.~Ito}{\AFFicrr}, 
\name{J.~Kameda}{\AFFicrr,\AFFipmu},
\name{Y.~Kataoka}{\AFFicrr},
\name{Y.~Kato}{\AFFicrr},
\name{Y.~Kishimoto}{\AFFicrr,\AFFipmu},
\name{M.~Miura} {\AFFicrr},
\name{S.~Moriyama}{\AFFicrr,\AFFipmu},
\name{T.~Mochizuki}{\AFFicrr},
\name{Y.~Nagao}{\AFFicrr},
\name{M.~Nakahata}{\AFFicrr,\AFFipmu},
\name{Y.~Nakajima}{\AFFicrr,\AFFipmu},
\name{S.~Nakayama}{\AFFicrr,\AFFipmu},
\name{T.~Okada}{\AFFicrr},
\name{K.~Okamoto}{\AFFicrr},
\name{G.~Pronost}{\AFFicrr},
\name{H.~Sekiya}{\AFFicrr,\AFFipmu},
\name{M.~Shiozawa}{\AFFicrr,\AFFipmu}, 
\name{Y.~Sonoda}{\AFFicrr},
\name{Y.~Suzuki}{\AFFicrr},
\name{A.~Takeda}{\AFFicrr,\AFFipmu},
\name{Y.~Takemoto}{\AFFicrr},
\name{A.~Takenaka}{\AFFicrr}, 
\name{H.~Tanaka}{\AFFicrr}, 
\name{T.~Yano}{\AFFicrr}, 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Kashiwa
\name{S.~Han}{\AFFkashiwa},
\name{T.~Kajita}{\AFFkashiwa,\AFFipmu},
\name{K.~Okumura}{\AFFkashiwa,\AFFipmu},
\name{T.~Tashiro}{\AFFkashiwa},
\name{R.~Wang}{\AFFkashiwa},
\name{J.~Xia}{\AFFkashiwa},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%ICRR kashiwa
\name{G.~D.~Megias}{\AFFicrrkashiwa},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Madrid
\name{D.~Bravo-Bergu\~{n}o}{\AFFmad},
\name{L.~Labarga}{\AFFmad},
\name{Ll.~Marti}{\AFFmad},
\name{B.~Zaldivar}{\AFFmad},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Boston U
\name{F.~d.~M.~Blaszczyk}{\AFFbu},
\name{E.~Kearns}{\AFFbu,\AFFipmu},
\name{J.~L.~Raaf}{\AFFbu},
\name{J.~L.~Stone}{\AFFbu,\AFFipmu},
\name{L.~Wan}{\AFFbu},
\name{T.~Wester}{\AFFbu},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% BCIT
\name{B.~W.~Pointon}{\AFFbcit},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Irvine
\name{J.~Bian}{\AFFuci},
\name{N.~J.~Griskevich}{\AFFuci},
\name{W.~R.~Kropp}{\AFFuci},
\name{S.~Locke}{\AFFuci},
\name{S.~Mine}{\AFFuci},
\name{M.~B.~Smy}{\AFFuci,\AFFipmu},
\name{H.~W.~Sobel}{\AFFuci,\AFFipmu},
\name{V.~Takhistov}{\AFFuci,\AFFipmu}%\thanks{also at Department of Physics and Astronomy, UCLA, CA 90095-1547, USA.},
\name{P.~Weatherly}{\AFFuci},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%CSU
\name{K.~S.~Ganezer}{\AFFcsu}\thanks{Deceased.},
\name{J.~Hill}{\AFFcsu},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Chonnam
\name{J.~Y.~Kim}{\AFFcnm},
\name{I.~T.~Lim}{\AFFcnm},
\name{R.~G.~Park}{\AFFcnm},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Duke
\name{B.~Bodur}{\AFFduke},
\name{K.~Scholberg}{\AFFduke,\AFFipmu},
\name{C.~W.~Walter}{\AFFduke,\AFFipmu},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%LLR
\name{L.~Bernard}{\AFFllr},
\name{A.~Coffani}{\AFFllr},
\name{O.~Drapier}{\AFFllr},
\name{S.~El Hedri}{\AFFllr},
\name{A.~Giampaolo}{\AFFllr},
\name{M.~Gonin}{\AFFllr},
\name{Th.~A.~Mueller}{\AFFllr},
\name{P.~Paganini}{\AFFllr},
\name{B.~Quilain}{\AFFllr},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Fukuoka
\name{T.~Ishizuka}{\AFFfukuoka},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Gifu U
\name{T.~Nakamura}{\AFFgifu},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Gwangju
\name{J.~S.~Jang}{\AFFgist},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Hawaii U
\name{J.~G.~Learned}{\AFFuh},
\name{S.~Matsuno}{\AFFuh},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%ICL
\name{L.~H.~V.~Anthony}{\AFFicl},
\name{R.~P.~Litchfield}{\AFFicl},
\name{A.~A.~Sztuc}{\AFFicl},
\name{Y.~Uchida}{\AFFicl},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%BARI
\name{V.~Berardi}{\AFFbari},
\name{M.~G.~Catanesi}{\AFFbari},
\name{E.~Radicioni}{\AFFbari},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%NAPOLI
\name{N.~F.~Calabria}{\AFFnapoli},
\name{L.~N.~Machado}{\AFFnapoli},
\name{G.~De Rosa}{\AFFnapoli},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%PADOVA
\name{G.~Collazuol}{\AFFpadova},
\name{F.~Iacob}{\AFFpadova},
\name{M.~Lamoureux}{\AFFpadova},
\name{N.~Ospina}{\AFFpadova},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Roma
\name{L.\,Ludovici}{\AFFroma},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Keio
\name{Y.~Nishimura}{\AFFkeio},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%KEK
\name{S.~Cao}{\AFFkek},
\name{M.~Friend}{\AFFkek},
\name{T.~Hasegawa}{\AFFkek},
\name{T.~Ishida}{\AFFkek},
\name{T.~Kobayashi}{\AFFkek},
\name{M.~Jakkapu}{\AFFkek},
\name{T.~Matsubara}{\AFFkek},
\name{T.~Nakadaira}{\AFFkek}, 
\name{K.~Nakamura}{\AFFkek,\AFFipmu},
\name{Y.~Oyama}{\AFFkek},
\name{K.~Sakashita}{\AFFkek},
\name{T.~Sekiguchi}{\AFFkek}, 
\name{T.~Tsukamoto}{\AFFkek}, 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%
%%KCL
\name{T.~Boschi}{\AFFkcl},
\name{F.~Di Lodovico}{\AFFkcl},
\name{S.~Molina Sedgwick}{\AFFkcl}\thanks{currently at Queen Mary University of London, London, E1 4NS, United Kingdom.},
\name{M.~Taani}{\AFFkcl}\thanks{also at School of Physics and Astronomy, University of Edinburgh, Edinburgh, EH9 3FD, United Kingdom},
\name{S.~Zsoldos}{\AFFkcl},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Kobe U
\name{M.~Hasegawa}{\AFFkobe},
\name{Y.~Isobe}{\AFFkobe},
\name{H.~Miyabe}{\AFFkobe},
\name{Y.~Nakano}{\AFFkobe},
\name{T.~Shiozawa}{\AFFkobe},
\name{T.~Sugimoto}{\AFFkobe},
\name{A.~T.~Suzuki}{\AFFkobe},
\name{Y.~Takeuchi}{\AFFkobe,\AFFipmu},
\name{S.~Yamamoto}{\AFFkobe},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Kyoto
\name{A.~Ali}{\AFFkyoto},
\name{Y.~Ashida}{\AFFkyoto},
\name{J.~Feng}{\AFFkyoto},
\name{S.~Hirota}{\AFFkyoto},
\name{M.~Jiang}{\AFFkyoto},
\name{A.~K.~Ichikawa}{\AFFkyoto},
\name{T.~Kikawa}{\AFFkyoto},
\name{M.~Mori}{\AFFkyoto},
\name{KE.~Nakamura}{\AFFkyoto},
\name{T.~Nakaya}{\AFFkyoto,\AFFipmu},
\name{R.~A.~Wendell}{\AFFkyoto,\AFFipmu},
\name{K.~Yasutome}{\AFFkyoto},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Liverpool
\name{P.~Fernandez}{\AFFliv},
\name{N.~McCauley}{\AFFliv},
\name{P.~Mehta}{\AFFliv},
\name{A.~Pritchard}{\AFFliv},
\name{K.~M.~Tsui}{\AFFliv},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Miyagi
\name{Y.~Fukuda}{\AFFmiyagi},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Nagoya
\name{Y.~Itow}{\AFFnagoya,\AFFkmi},
\name{H.~Menjo}{\AFFnagoya},
\name{T.~Niwa}{\AFFnagoya},
\name{K.~Sato}{\AFFnagoya},
\name{M.~Tsukada}{\AFFnagoya},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% POLAND
\name{P.~Mijakowski}{\AFFpol},
\name{K.~Frankiewicz}{\AFFpol},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%SUNY
\name{C.~K.~Jung}{\AFFsuny},
\name{C.~Vilela}{\AFFsuny},
\name{M.~J.~Wilking}{\AFFsuny},
\name{C.~Yanagisawa}{\AFFsuny}\thanks{also at BMCC/CUNY, Science Department, New York, New York, USA.},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Okayama U
\name{D.~Fukuda}{\AFFokayama},
\name{M.~Harada}{\AFFokayama},
\name{K.~Hagiwara}{\AFFokayama},
\name{T.~Horai}{\AFFokayama},
\name{H.~Ishino}{\AFFokayama},
\name{S.~Ito}{\AFFokayama},
\name{Y.~Koshio}{\AFFokayama,\AFFipmu},
\name{W.~Ma}{\AFFokayama},
\name{N.~Piplani}{\AFFokayama},
\name{S.~Sakai}{\AFFokayama},
\name{M.~Sakuda}{\AFFokayama},
\name{Y.~Takahira}{\AFFokayama},
\name{C.~Xu}{\AFFokayama},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Osaka U.
\name{Y.~Kuno}{\AFFosaka},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Oxford
\name{G.~Barr}{\AFFox},
\name{D.~Barrow}{\AFFox},
\name{L.~Cook}{\AFFox,\AFFipmu},
\name{A.~Goldsack}{\AFFox,\AFFipmu},
\name{S.~Samani}{\AFFox},
\name{C.~Simpson}{\AFFox,\AFFipmu},
\name{D.~Wark}{\AFFox,\AFFstfc},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Queen Mary
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%RAL
\name{F.~Nova}{\AFFral},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Seoul
\name{J.~Y.~Yang}{\AFFseoul},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Sheffield
\name{S.~J.~Jenkins}{\AFFsheff},
\name{M.~Malek}{\AFFsheff},
\name{J.~M.~McElwee}{\AFFsheff},
\name{O.~Stone}{\AFFsheff},
\name{M.~D.~Thiesse}{\AFFsheff},
\name{L.~F.~Thompson}{\AFFsheff},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Shizuoka Seika College
\name{H.~Okazawa}{\AFFshizuokasc},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%SungKyunKwan
\name{Y.~Choi}{\AFFskk},
\name{S.~B.~Kim}{\AFFskk},
\name{I.~Yu}{\AFFskk},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Tokai U
\name{K.~Nishijima}{\AFFtokai},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Tokyo
\name{M.~Koshiba}{\AFFtokyo}\thanks{Deceased.},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Tokyo, Deartment of Physics
\name{K.~Iwamoto}{\AFFtodai},
\name{N.~Ogawa}{\AFFtodai},
\name{M.~Yokoyama}{\AFFtodai,\AFFipmu},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%IPMU
\name{K.~Martens}{\AFFipmu},
\name{M.~R.~Vagins}{\AFFipmu,\AFFuci},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%TIT
\name{S.~Izumiyama}{\AFFtit},
\name{M.~Kuze}{\AFFtit},
\name{M.~Tanaka}{\AFFtit},
\name{T.~Yoshida}{\AFFtit},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%TUS
\name{M.~Inomoto}{\AFFtus},
\name{M.~Ishitsuka}{\AFFtus},
\name{R.~Matsumoto}{\AFFtus},
\name{K.~Ohta}{\AFFtus},
\name{M.~Shinoki}{\AFFtus},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Toronto
\name{J.~F.~Martin}{\AFFtoronto},
\name{C.~M.~Nantais}{\AFFtoronto},
\name{H.~A.~Tanaka}{\AFFtoronto},
\name{T.~Towstego}{\AFFtoronto},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Triumf
\name{R.~Akutsu}{\AFFtriumf},
\name{M.~Hartz}{\AFFtriumf,\AFFipmu},
\name{A.~Konaka}{\AFFtriumf},
\name{P.~de Perio}{\AFFtriumf},
\name{N.~W.~Prouse}{\AFFtriumf},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Tshinghua U
\name{S.~Chen}{\AFFtsinghua},
\name{B.~D.~Xu}{\AFFtsinghua},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Warsaw
\name{M.~Posiadala-Zezula}{\AFFwu},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Warwick
\name{B.~Richards}{\AFFwarwick},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Winnipeg
\name{B.~Jamieson}{\AFFwinnipeg},
\name{J.~Walker}{\AFFwinnipeg},
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Yokohama
\name{A.~Minamino}{\AFFynu},
\name{K.~Okamoto}{\AFFynu},
\name{G.~Pintaudi}{\AFFynu},
\name{R.~Sasaki}{\AFFynu},
%\name{(The Super-Kamiokande Collaboration)}{}}
\collaborator{(The Super-Kamiokande Collaboration)}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\address{
\affil[\AFFicrr]{{Kamioka Observatory, Institute for Cosmic Ray Research, University of Tokyo, Kamioka, Gifu 506-1205, Japan}}
\affil[\AFFkashiwa]{{Research Center for Cosmic Neutrinos, Institute for Cosmic Ray Research, University of Tokyo, Kashiwa, Chiba 277-8582, Japan}}
\affil[\AFFicrrkashiwa]{{Institute for Cosmic Ray Research, University of Tokyo, Kashiwa, Chiba 277-8582, Japan}}
\affil[\AFFmad]{{Department of Theoretical Physics, University Autonoma Madrid, 28049 Madrid, Spain}}
\affil[\AFFbu]{{Department of Physics, Boston University, Boston, MA 02215, USA}}
\affil[\AFFbcit]{{Department of Physics, British Columbia Institute of Technology, Burnaby, BC, V5G 3H2, Canada }}
\affil[\AFFuci]{{Department of Physics and Astronomy, University of California, Irvine, Irvine, CA 92697-4575, USA }}
\affil[\AFFcsu]{{Department of Physics, California State University, Dominguez Hills, Carson, CA 90747, USA}}
\affil[\AFFcnm]{{Institute for Universe and Elementary Particles, Chonnam National University, Gwangju 61186, Korea}}
\affil[\AFFduke]{{Department of Physics, Duke University, Durham NC 27708, USA}}
\affil[\AFFllr]{{Ecole Polytechnique, IN2P3-CNRS, Laboratoire Leprince-Ringuet, F-91120 Palaiseau, France }}
\affil[\AFFfukuoka]{{Junior College, Fukuoka Institute of Technology, Fukuoka, Fukuoka 811-0295, Japan}}
\affil[\AFFgifu]{{Department of Physics, Gifu University, Gifu, Gifu 501-1193, Japan}}
\affil[\AFFgist]{{GIST College, Gwangju Institute of Science and Technology, Gwangju 500-712, Korea}}
\affil[\AFFuh]{{Department of Physics and Astronomy, University of Hawaii, Honolulu, HI 96822, USA}}
\affil[\AFFicl]{{Department of Physics, Imperial College London , London, SW7 2AZ, United Kingdom }}
\affil[\AFFbari]{{ Dipartimento Interuniversitario di Fisica, INFN Sezione di Bari and Universit\`a e Politecnico di Bari, I-70125, Bari, Italy}}
\affil[\AFFnapoli]{{Dipartimento di Fisica, INFN Sezione di Napoli and Universit\`a di Napoli, I-80126, Napoli, Italy}}
\affil[\AFFpadova]{{Dipartimento di Fisica, INFN Sezione di Padova and Universit\`a di Padova, I-35131, Padova, Italy}}
\affil[\AFFroma]{{INFN Sezione di Roma and Universit\`a di Roma ``La Sapienza'', I-00185, Roma, Italy}}
\affil[\AFFkeio]{{Department of Physics, Keio University, Yokohama, Kanagawa, 223-8522, Japan}}
\affil[\AFFkek]{{High Energy Accelerator Research Organization (KEK), Tsukuba, Ibaraki 305-0801, Japan }}
\affil[\AFFkcl]{{Department of Physics, King's College London, London, WC2R 2LS, UK }}
\affil[\AFFkobe]{{Department of Physics, Kobe University, Kobe, Hyogo 657-8501, Japan}}
\affil[\AFFkyoto]{{Department of Physics, Kyoto University, Kyoto, Kyoto 606-8502, Japan}}
\affil[\AFFliv]{{Department of Physics, University of Liverpool, Liverpool, L69 7ZE, United Kingdom}}
\affil[\AFFmiyagi]{{Department of Physics, Miyagi University of Education, Sendai, Miyagi 980-0845, Japan}}
\affil[\AFFnagoya]{{Institute for Space-Earth Environmental Research, Nagoya University, Nagoya, Aichi 464-8602, Japan}}
\affil[\AFFkmi]{{Kobayashi-Maskawa Institute for the Origin of Particles and the Universe, Nagoya University, Nagoya, Aichi 464-8602, Japan}}
\affil[\AFFpol]{{National Centre For Nuclear Research, 02-093 Warsaw, Poland}}
\affil[\AFFsuny]{{Department of Physics and Astronomy, State University of New York at Stony Brook, NY 11794-3800, USA}}
\affil[\AFFokayama]{{Department of Physics, Okayama University, Okayama, Okayama 700-8530, Japan }}
\affil[\AFFosaka]{{Department of Physics, Osaka University, Toyonaka, Osaka 560-0043, Japan}}
\affil[\AFFox]{{Department of Physics, Oxford University, Oxford, OX1 3PU, United Kingdom}}
\affil[\AFFqmul]{{School of Physics and Astronomy, Queen Mary University of London, London, E1 4NS, United Kingdom}}
\affil[\AFFral]{{Rutherford Appleton Laboratory, Harwell, Oxford, OX11 0QX, UK }}
\affil[\AFFseoul]{{Department of Physics, Seoul National University, Seoul 151-742, Korea}}
\affil[\AFFsheff]{{Department of Physics and Astronomy, University of Sheffield, S3 7RH, Sheffield, United Kingdom}}
\affil[\AFFshizuokasc]{{Department of Informatics in Social Welfare, Shizuoka University of Welfare, Yaizu, Shizuoka, 425-8611, Japan}}
\affil[\AFFstfc]{{STFC, Rutherford Appleton Laboratory, Harwell Oxford, and Daresbury Laboratory, Warrington, OX11 0QX, United Kingdom}}
\affil[\AFFskk]{{Department of Physics, Sungkyunkwan University, Suwon 440-746, Korea}}
\affil[\AFFtokai]{{Department of Physics, Tokai University, Hiratsuka, Kanagawa 259-1292, Japan}}
\affil[\AFFtokyo]{{The University of Tokyo, Bunkyo, Tokyo 113-0033, Japan }}
\affil[\AFFtodai]{{Department of Physics, University of Tokyo, Bunkyo, Tokyo 113-0033, Japan }}
\affil[\AFFipmu]{{Kavli Institute for the Physics and Mathematics of the Universe (WPI), The University of Tokyo Institutes for Advanced Study, University of Tokyo, Kashiwa, Chiba 277-8583, Japan }}
\affil[\AFFtit]{{Department of Physics,Tokyo Institute of Technology, Meguro, Tokyo 152-8551, Japan }}
\affil[\AFFtus]{{Department of Physics, Faculty of Science and Technology, Tokyo University of Science, Noda, Chiba 278-8510, Japan }}
\affil[\AFFtoronto]{{Department of Physics, University of Toronto, ON, M5S 1A7, Canada }}
\affil[\AFFtriumf]{{TRIUMF, 4004 Wesbrook Mall, Vancouver, BC, V6T2A3, Canada }}
\affil[\AFFtsinghua]{{Department of Engineering Physics, Tsinghua University, Beijing, 100084, China}}
\affil[\AFFwu]{{Faculty of Physics, University of Warsaw, Warsaw, 02-093, Poland }}
\affil[\AFFwarwick]{{Department of Physics, University of Warwick, Coventry, CV4 7AL, UK }}
\affil[\AFFwinnipeg]{{Department of Physics, University of Winnipeg, MB R3J 3L8, Canada }}
\affil[\AFFynu]{{Department of Physics, Yokohama National University, Yokohama, Kanagawa, 240-8501, Japan}}

